2-Segal objects and algebras in spans

We define a category parameterizing Calabi-Yau algebra objects in an infinity category of spans. Using this category, we prove that there are equivalences of infinity categories relating, firstly: 2-Segal simplicial objects in C to algebra objects in Span(C); and secondly: 2-Segal cyclic objects in C to Calabi-Yau algebra objects in Span(C).

==> menagerie.tex <==
\section{The menagerie: notations, background, and constructions}

In this section, we will lay out the fundamental definitions and constructions that will be used in the proof of the main result. Along the way, we will also prove basic relations between these definitions, to alleviate the density of later arguments.
\subsection{Linear and cyclic orders}
\begin{defn}\label{defn:SimplexCats}
The \emph{simplex category} $\Delta$ has objects the standard linearly ordered sets $[n]=\{0,1,\ldots, n\}$ for $n\geq 0$ and morphisms the order-preserving maps. The \emph{enlarged simplex category} $\bbDelta$ has objects finite non-empty linearly ordered sets, and morphisms order-preserving maps. 

The \emph{augmented simplex category} $\Delta_+$ (resp. the \emph{augmented simplex category} $\bbDelta_+$) is obtained from  $\Delta$ (resp. $\bbDelta$) by appending an initial object $\emptyset$, which will also sometimes be denoted by $[-1]$.

The \emph{interval category} $\nabla$ is the subcategory of $\Delta$ on the objects $[n]$ for $n\geq 1$, the morphisms of which preserve maximal and minimal elements. The \emph{enlarged interval category} $\bbNabla$ is the subcategory of $\bbDelta$ on those sets of cardinality $\geq 2$, whose morphisms preserve maximal and minimal elements.

The \emph{augmented interval category} $\nabla_+$ (resp. the \emph{augmented extended interval category} $\bbNabla_+$) is the subcategory of $\Delta$ (resp. $\bbDelta$) whose objects have cardinality $\geq 1$ and whose morphisms preserve the maximal and minimal elements. 
\end{defn}

We denote by $S^1$ the unit circle $\{z\in \mathbb{C}|\,|z|=1\}$, and equip it with the orientation inherited from $\mathbb{C}$. We will denote by $r(n)=\{e^{\frac{2\pi i k}{n+1}}|0\leq k<n+1\}$ the sets of roots of unity in $S^1$. {\color{red} define cyclic orders}

\begin{defn}\label{defn:CyclicCats}
The \emph{cyclic category} has as its objects the standard cyclicly ordered sets $\langle n\rangle$ for $n\geq 0$, and as its morphisms the maps of finite sets respecting the cyclic order. The \emph{enlarged cyclic category} $\bbLambda$ has as its objects all finite, non-empty, cyclicly ordered sets, and as its morphisms the maps which respect the cyclic order.
\end{defn}

\begin{defn}\label{defn:SetCats}
The category of the standard finite sets $\underline{n}:=\{1,2,\ldots, n\}$ for $n\geq 0$ will be denoted $\Fin$. The category of the standard finite pointed sets $\langle n\rangle:=\underline{n}\amalg \{\ast\}$ will be denoted $\Fin_\ast$. The category of all finite sets (resp. the category of all finite points sets) will be denoted by $\bFin$ (resp. by $\bFin_\ast$). When convenient, we will denote by $\bbGamma$ (resp. by $\Gamma$) the opposites of the categories $\bFin_\ast$ (resp. $\Fin_\ast$). 

We additionally denote by $\Ass$ the associative operad\todo{expand this defn}. 

Given a pointed set $S\in \bFin_\ast$, we denote by $S^\circ$ the set $S\setminus \{\ast\}$, where $\ast$ denotes the basepoint of $S$. 
\end{defn}

\begin{const}[Linear interstices]\label{const:LinInterstice}
Given a linearly ordered set $S\in \bbDelta$ we define an \emph{inner interstice} of $S$ to be an ordered pair $(k,k+1)\in S\times S$, where $k+1$ denotes the successor to $k$. The set of inner interstices of $S$ is, itself, a linearly ordered set, with the order
\[
(k,k+1)\leq (j,j+1)\Leftrightarrow k\leq j
\]
We will denote the linearly ordered set of inner interstices of $S$ by $\mathbb{I}(S)$. Note that $\mathbb{I}([0])=\emptyset$. 

Given a linearly ordered set $S\in \bbDelta_+$, let $\hat{S}$ be the set $\{a\}\amalg S\amalg \{b\}$, where $b$ is taken to be maximal and $a$ minimal. We define an \emph{outer interstice} of $S$ to be an inner interstice of $\hat{S}$. We will denote the linearly ordered set of outer interstices of $S$ by $\mathbb{O}(S)$. Note that $\mathbb{O}(\emptyset)=\{(a,b)\}$. 

We define functors 
\[
\mathbb{O}:\bbDelta_+^{\op}\to \bbNabla_+;\quad S\mapsto \mathbb{O}(S)
\]
and 
\[
\mathbb{I}: \bbNabla_+^\op\to \bbDelta;\quad S\mapsto \mathbb{I}(S)
\]
as follows (we will define $\mathbb{O}$ explicitly, the definition of $\mathbb{I}$ is similar). Given a morphism $f:S\to T$ in $\bbDelta_+$, we define a morphism $\mathbb{O}(f):\mathbb{O}(S)\to \mathbb{O}(T)$ by setting 
\[
\mathbb{O}(f)(j,j+1)=\begin{cases}
				 	(k,k+1) & f(k)\leq j\leq j+1\leq f(k+1)\\
				 	(a,a+1) & j\leq f(k)\; \forall k\in S\\
				 	(b-1,b) & j\geq f(k)\; \forall k\in S. 
				 \end{cases}
\]
Pictorially, we can represent the morphism $\mathbb{O}(f)$ as a forest as in Figure \ref{fig:DualForest}, thinking leaves $j\in \mathbb{O}(T)$ as being attached to the root $k\in \mathbb{O}(S)$ if $\mathbb{O}(f)(j)=k$. 
\begin{figure}[htb]
\begin{tikzpicture}
\foreach \x/\lab/\nom in {0.5/a_0/a0,1.5/a_1/a1,2.5/a_2/a2,3.5/a_3/a3}{
\path (0,-\x) node (\nom) {$\lab$}; 
};
\begin{scope}[yshift=12]
\foreach \x/\lab/\nom in {0.5/b_0/b0,1.5/b_1/b1,2.5/b_2/b2,3.5/b_3/b3,4.5/b_4/b4}{
\path (4,-\x) node (\nom) {$\lab$}; 
};
\end{scope}
\draw[->] (a0) to (b0);
\draw[->] (a1) to (b2);
\draw[->] (a2) to (b3);
\draw[->] (a3) to (b3);
\end{tikzpicture}
\qquad
\begin{tikzpicture}
\foreach \x/\lab/\nom in {0.5/a_0/a0,1.5/a_1/a1,2.5/a_2/a2,3.5/a_3/a3}{
\path (0,-\x) node (\nom) {$\lab$}; 
};
\foreach \y in {0,1,2,3,4}{
\draw[blue](-0.2,-\y) to (0.2,-\y); 
};
\begin{scope}[yshift=12]
\foreach \x/\lab/\nom in {0.5/b_0/b0,1.5/b_1/b1,2.5/b_2/b2,3.5/b_3/b3,4.5/b_4/b4}{
\path (4,-\x) node (\nom) {$\lab$}; 
};
\foreach \y in {0,1,2,3,4,5}{
\draw[blue](4.2,-\y) to (3.8,-\y); 
}
\end{scope}
\draw[->] (a0) to (b0);
\draw[->] (a1) to (b2);
\draw[->] (a2) to (b3);
\draw[->] (a3) to (b3);
\end{tikzpicture}
\caption{Left: a morphism $f$ of linearly ordered sets. Right: the morphism $\mathbb{O}(f)$, visualized as a forest (blue). {\color{red} Finish!!!}}\label{fig:DualForest}
\end{figure}  

Note that the functors $\mathbb{I}$ and $\mathbb{O}$ define an equivalence of categories. Since $\Delta_+$ (resp. $\nabla_+$) is the skeletal version of $\bbDelta_+$ (resp. $\bbNabla_+$), and is gaunt, we see that we get an induced \emph{isomorphism} of categories
\[
O:\Delta_+^\op\overset{\cong}{\longleftrightarrow }\nabla_+:I
\] 
Moreover, we can define a functor $\bbNabla_+\to \Fin_\ast$ by 
\[
S\mapsto (S\amalg \{\ast\})_{/\on{max}(S)\sim\on{min}(s)\sim \ast}
\]
We then find that the induced functor 
\[
\Delta_+^{\op}\hookrightarrow \Delta_+^\op\overset{O}{\to} \nabla_+\to \Fin_\ast
\]
is precisely the functor $\on{cut}:\Delta^\op\to \Fin_\ast$ defined in \cite[4.1.2.9]{LurieHA}.
\end{const}

\begin{defn}
Given two linearly ordered sets $S,T\in \bbDelta_+$ define the \emph{ordinal sum} $S\oplus T$ to be the set $S\amalg T$ equipped with the linear order defined by the orders on $S$ and $T$ and the proscription that for all $s\in S$ and $t\in T$, $s\leq t$. The ordinal sum defines a monoidal structure on $\bbDelta_+$. 

Given two linearly ordered sets $S,T\in \bbNabla_+$, with $b$ the maximum of $S$ and $a$ the minimum of $T$, define the \emph{imbrication} $S\star T$ to be the linearly ordered set $(S\oplus T)_{/a\sim b}$ (note that since $a$ is the successor to $b$ in $S\oplus T$, there is a canonical linear order on $S\star T$ compatible with the quotient map). 
\end{defn}

\begin{lem}
The functor $\mathbb{O}$ is a monoidal functor sending the ordinal sum to the imbrication. 
\end{lem}
\begin{proof}
The\todo{add?} 
\end{proof}


\begin{const}[Cyclic Duality]\label{const:CyclicDuality}
In analogy to the construction of the linear interstice functors, we define a duality  
\[
\mathbb{D}:\bbLambda^{\op}\to \bbLambda
\]
on the cyclic category. Let $S\in \bbLambda$ be a cyclicly ordered set. We define a \emph{cyclic interstice} of $S$ to be an ordered pair $(a,a+1)\in S\times S$, where $a+1$ denotes the successor of $a$ under the cyclic order. We denote the set of cyclic interstices of $S$ by $\mathbb{D}(S)$. The set $\mathbb{D}(S)$ inherits a canonical cyclic order from $S$\todo{give explicit characterization}, which can be visualized as in Figure \ref{fig:CyclicInterstices}. 
\begin{figure}[htb]
\begin{tikzpicture}
\draw (0,0) circle (1);
\foreach \th in {0,60,120,180,240,300}{
\draw[fill=black] (\th:1) circle (0.05);
};
\foreach \th in {30,90,150,210,270,330}{
\draw[blue,fill=blue] (\th:1) circle (0.05);
};
\end{tikzpicture}
\caption{A cyclic set with its cyclic order visualized via an embedding into the oriented circle (black), together with its set of cyclic interstices (blue).}\label{fig:CyclicInterstices}
\end{figure}
The functor $\mathbb{D}$ is specified on morphisms by an analogue of \ref{const:LinInterstice}, namely, for $f:S\to T$ in $\bbLambda$, we set\todo{Give explicit characterization}
\[
\mathbb{D}(f)(j,j+1):=k\quad \text{where }  
\]
This functor is an equivalence of categories\todo{Cite DK}.
Since $\Lambda$ is the skeletal version of $\bbLambda$, $\mathbb{D}$ descends to an equivalence $D:\Lambda^\op\to \Lambda$
\end{const}


\begin{const}[Cyclic closures]\label{const:CyclicClosures}
We define a functor $\mathbb{K}:\bbDelta\to \bbLambda$ in the following way. Given a linearly ordered set $S$ of cardinality $n+1$, there is a unique order-preserving bijection $\phi:S\to [n]$. We define a bijection 
\[
S\to r(n); \quad j\mapsto \exp\left(\frac{2\pi i \phi(j)}{n+1}\right) 
\]
to the $n^{\on{th}}$ roots of unity in $S^1$. The orientation on $S^1$ then yields a canonical cyclic order on $S$. \todo{on morphisms} Passing to skeletal versions yields the well-known functor $\kappa: \Delta\to \Lambda$. 

Via the equivalences $\mathbb{O}$ and $\mathbb{D}$ we can then define a functor $\mathbb{C}:\bbNabla\to \Lambda$ such that the diagram 
\[
\begin{tikzcd}
\bbDelta^\op\arrow[d,"\mathbb{K}"']\arrow[r,"\mathbb{O}"] & \bbNabla\arrow[d,"\mathbb{C}"]\\
\bbLambda^\op\arrow[r,"\mathbb{D}"'] & \bbLambda
\end{tikzcd}
\]
commutes up to natural isomorphism. The functor $\mathbb{C}$ admits the following explicit description on objects. Let $S\in \bbNabla$ with maximal element $b$ and minimal element $a$. Then $\mathbb{C}(S)$ can be identified with with quotient of $\mathbb{K}(S)$ by the identification $a\sim b$.\todo{write about cyclic order here} Once again, we have that $\mathbb{C}$ descends to a functor $C:\nabla\to \Lambda$. 
\end{const}

\begin{defn}\label{defn:CyclicCatChosenTriv}
We introduce one final equivalent variant of $\bbLambda$, which we will denote $\bfLambda$. The objects of $\bfLambda$ consist of pairs $(S,\phi)$ where $S\in \bbLambda$, and $\phi:S\to \langle |S|-1\rangle$ is an isomorphism in $\bbLambda$. The morphisms of $S$ are simply the morphisms of $\bbLambda$.  It is clear that the forgetful functor $\bfLambda\to\bbLambda$ is an equivalence. 
\end{defn}

\subsection{Calabi-Yau algebras}

\begin{defn}
We define a category $\Ass_\CY$ to have objects given by $S\in \bFin_\ast$ together with a partition $S_1\amalg S_2=S^\circ$. We will denote these objects by the ordered pair $\langle S_1,S_2\rangle$. A morphism $\langle S_1,S_2\rangle\to \langle T_1,T_2\rangle$ consists of 
\begin{enumerate}
\item A morphism $\phi:S\to T$ in $\bFin_\ast$ such that, for every $i\in T$ such that $\phi^{-1}(i)\neq \emptyset$
\begin{itemize}
\item for every $i\in T_1$, $\phi^{-1}(i)\subset S_1$
\item for every $i\in T_2$, either $\phi^{-1}(i)\subset S_1$ or $\phi^{-1}(i)\in S_2$ is a single element. 
\end{itemize}
\item If $i\in T_1$, a linear order on $\phi^{-1}(i)$.
\item If $i\in T_2$ with $\phi^{-1}(i)\subset S_1$, a cyclic order on $\phi^{-1}(i)$. 
\end{enumerate}
Composition in $\Ass_\CY$ is defined by composition in $\bFin_\ast$, together with the induced linear and cyclic orders. \todo{Write whole up} Note that $\Ass_\CY$ comes equipped with a forgetful functor to $\bFin_\ast$. 
\end{defn}

\begin{lem}
The functor $\Ass_\CY\to \bFin_\ast$ displays $\Ass_\CY$ as an $\infty$-operad. 
\end{lem}

\begin{proof}
We first note that if $\phi:S\to T$ is an inert morphism in $\bFin_\ast$ and $\langle S_1,S_2\rangle$ is an object in $\Ass_\CY$ lying over $S$, we can define $T_1:=\phi(S_1)$ and $T_2=\phi(S_2)$ to get an object $\langle T_1,T_2\rangle$ over $T$. Since $\phi$ is inert, we need specify no extra data to lift $\phi$ to a morphism $\tilde{\phi}:\langle S_1,S_2\rangle \to \langle T_1,T_2\rangle$. 

Let $\tilde{\psi}: \langle S_1,S_2\rangle \to \langle U_1,U_2\rangle$ be any morphism in $\Ass_\CY$, and let $\psi:S\to U$ be its image in $\bFin_\ast$. Suppose $\gamma:T\to U$ is a morphism in $\bFin_\ast$    
\end{proof}

\subsection{Cartesian monoidal structures}

Throughout this paper, we will model (symmetric) monoidal structions by Cartesian fibrations, rather than the coCartesian fibrations used in \cite{LurieHA}. These fibrations will be defined via adjunctions with the following. Throughout this section, $\CC$ will denote an $\infty$-category which admits finite products. 

\begin{defn}
The category $\Delta^{\amalg}$ has as its objects  pairs $([n],\{i,j\})$, where $[n]\in \Delta$ and $i\leq j$ are elements in $[n]$. The morphisms $ ([n],\{i,j\})\to ([m],\{k,\ell\})$ consist of a morphism $\phi:[n]\to [m]$ such that $\phi(i)\leq k\leq \ell\leq \phi(j)$.  We will, in general, think of $\{i,j\}$ as an interval inside $[n]$, and denote by $\{i\leq j\}$ the linearly ordered set 
\[
\{i\leq j\}:= \{i,i+1,\ldots,j\}\subset [n].
\]

The category $\bFin_\ast^\amalg$ has as its objects pairs $(S, T)$ where $S\in \bFin_\ast$ and $T\subset S^\circ$. A morphism $(S,T)\to (P,Q)$ consists of a morphism $\phi:S\to P$ in $\bFin_\ast$ such that $\phi(T)\subset Q$. We will sometimes denote by $\bbGamma^\amalg$ the category $(\bFin_\ast^\amalg)^\op$.   
\end{defn}

\begin{rmk}
We can provide an alternate characterization of $\Delta^\amalg$ and $(\bFin_\ast^\amalg)^\op$. They are the coCartesian fibrations defined as Grothendieck constructions of the functors\todo{provide definitions of $I_{[n]}$ etc.} 
\[
\Delta\to \Cat;\quad [n] \mapsto I_{[n]}^\op
\]
and the contravariant power set functor
\[
\bFin_\ast^\op\to \Cat;\quad S\mapsto \mathcal{P}(S^\circ)^\op
\]
respectively. 
\end{rmk}

\begin{const}
The functor $\on{cut}:\Delta\to \bFin_\ast^\op$ yields a functor $\Delta^\amalg\to (\bFin_\ast^\amalg)^\op$. To see this, we first note that for $\{i,j\}\subset [n]$ in $\Delta^\amalg$, we have $\mathbb{O}(\{i\leq j\})\subset \mathbb{O}([n])$. On objects we therefore define $\{i,j\}\subset [n]\mapsto (\mathbb{O}([n]),\mathbb{O}(\{i\leq j\}))$ 

Given a morphism $f:([n],\{i,j\})$ to $([m],\{k,\ell\})$ in $\Delta^\amalg$, we get a morphism $\mathbb{O}(f): \mathbb{O}([m])\to \mathbb{O}([n])$. Moreover, the condition that $f(i)\leq k\leq \ell\leq f(j)$ ensures that $\mathbb{O}(f)\left( \mathbb{O}(\{k\leq \ell\})\right) \subset \mathbb{O}(\{i\leq j\})$. 
\end{const}

\begin{const}[Cartesian monoidal structures]
Given an $\infty$-category $\CC$ with finite products, we can associate two Cartesian fibrations to $\CC$ as follows. 

We define a functor of $\infty$-categories $\overline{\CC^\boxtimes} \to \Delta$ via the universal property 
\[
\Hom_\Delta(K, \overline{\CC^\boxtimes})\cong \Hom_{\Set_\Delta} (K\times_\Delta \Delta^\amalg, \CC).
\]
Similarly, we define a functor $\overline{\CC^\times}\to \bbGamma$ via the universal property 
\[
\Hom_{\bbGamma}(K, \overline{\CC^\boxtimes})\cong \Hom_{\Set_\Delta} (K\times_{\bbGamma} \bbGamma^\amalg, \CC).
\]
Both of these are Cartesian fibrations by dint of \cite[3.2.2.13]{LurieHTT}.

We now let $\CC^\boxtimes\subset \overline{\CC^\boxtimes}$ be the full subcategory on those objects $G:I_[n]^\op\to \CC$ for which $G$ displays $G(\{i\leq j\})$ as a product over $G(\{k\leq k+1\})$ for $i\leq k<j$.

Similarly, we let $\CC^\times\subset \overline{\CC^\times}$ be the full subcategory on those objects $G:\mathcal{P}(S^\circ)^{\op}$ for which  $G$ displays $G(S)$ as a product over $G(i)$ for $i\in S$. \todo{FINISH!!}
\end{const}

\begin{prop}
The functor $\CC^\boxtimes\to \Delta$ is a Cartesian fibration exhibiting the Cartesian monoidal structure on $\CC$.
\end{prop}

\begin{proof}
This is \cite[Prop. 10.3.8]{DKHSSI}.
\end{proof}

\begin{prop}
The functor $\CC^\times\to \bbGamma$ is a Cartesian fibration exhibiting the Cartesian symmetric monoidal structure on $\CC$. 
\end{prop}

\begin{proof}
We first note that $\CC^\times\to \bbGamma$ is a\todo{Fill in. Mutatis mutandis same as in DKHSSI.}  
\end{proof}


\subsection{Categories of Spans}
Throughout this section, we will assume that $\CC$ is now an $\infty$-category with small limits. 

\begin{const}[Categories of Spans]\label{const:TwSpan}
We define the functor $\Tw:\Delta\to \Set_\Delta$ by 
\[
[n]\mapsto N(I_{[n]})^\op.
\]
By left Kan extension along the Yoneda embedding and restriction, we get an adjunction, which we will abuse notation and denote by
\[
\Tw:\Set_\Delta\leftrightarrow \Set_\Delta: \Span.
\]
For an $\infty$-category $\DD$, the simplicial set $\Tw(\DD)$ is an $\infty$-category, which we will call the \emph{twisted arrow $\infty$-category} of $\DD$. 

Given  $B\in \Set_\Delta$, we can   
\end{const}

==> scratch.tex <==
\begin{proof}
There are two cases to consider, corresponding to whether or not $S=\diamond$. 

\phantomsection
\label{proof:CaseOne}
{\itshape Case 1:} First suppose $S\in \Ass$. In this case, we construct $X_{M,Z}$ as follows. Let 
\[
P\subset P \overset{f_M}{\longleftarrow} U
\]
be the object constructed in \cref{prop:LambdaLaxFibOverAss}. Then, in particular, $\phi:P\to Q\subset S$. 

For each $i\in Q$, we have a morphism 
\[
\gamma_i: \bigoplus_{j\in \phi^{-1}(i)}[m_i]\to O(f_Z^{-1}(i))
\]
For each $j\in \phi^{-1}(i)$ denote by $\gamma_i([m_j])$ the smallest subinterval of $O(f_Z^{-1}(i))$ containing the image of $[m_j]$ under $\gamma_i$. Then $\gamma_i|_{[m_j]}\to \gamma_i([m_j])$ preserves boundary, and thus corresponds to a map $\overline{g}_{j}:I(\gamma_i([m_j]))\to I([m_j])$ of linearly ordered sets. Moreover, $\overline{g}_j$ fits into a commutative diagram 
\[
\begin{tikzcd}
S & I(\gamma_i([m_j]))\arrow[l,"f_{Z}"']\arrow[d,"\overline{g}_j"]\\
P\arrow[u,"\phi"] & I([m_j])\arrow[l,"f_M"']
\end{tikzcd}
\]
in $\Ass$. We here use the identification of  $I(\gamma_i([m_j]))$ with a subset of $T$. 

Since, by definition, $U=\coprod_{j\in P} I([m_j])$, we can then write down a commutative diagram 
\begin{equation}\label{diag:CommXZM}
\begin{tikzcd}
S & \coprod_{i,j}I(\gamma_i([m_j]))\arrow[l,"f_{Z}"']\arrow[d,"\coprod_{i,j}\overline{g}_j"]\\
P\arrow[u,"\phi"] & \coprod_{j\in P} I([m_j])\arrow[l,"f_M"']
\end{tikzcd}
\end{equation}
in $\Ass$. 

For each $i\in Q$, this restricts to a diagram of ordered sets 
\[
\begin{tikzcd}
\{i\} & \coprod_{j}I(\gamma_i([m_j]))\arrow[l,"f_{Z}"']\arrow[d,"\coprod_{j}\overline{g}_j"]\\
\phi^{-1}(i)\arrow[u,"\phi"] & \coprod_{j\in\phi^{-1}(i)} I([m_j])\arrow[l,"f_M"']
\end{tikzcd}
\]
We denote $L_i:=f_Z^{-1}(i)\setminus\coprod_{j\in \phi^{-1}(i)}I(\gamma_i([m_j])$, and proceed as follows.
\begin{itemize}
\item For $p, p+1$ in $\phi^{-1}(i)$, if there is at least one $k\in L_i$ such that
\[
I(\gamma_i([m_{p}]))<k< I(\gamma_i([m_{p+1}]))
\]
 we define a new element $r_p$ and append it to $\phi^{-1}(i)$ between $p$ and $p+1$.
\item If there exists $k\in L_i$ such that 
\[
k< I(\gamma_i([m_{p}]))
\]
for all $p\in \phi^{-1}(i)$, then we append a new minimal element $r_{min}$ to $\phi^{-1}(i)$. 
\item If there exists $k\in L_i$ such that 
\[
I(\gamma_i([m_{p}]))< k
\]
for all $p\in \phi^{-1}(i)$, then we append a new maximal element $ $ to $\phi^{-1}(i)$.
\end{itemize} 
Call the resulting set $W_i\supset \phi^{-1}(i)$. We then set 
\[
R_i:= U\amalg L_i
\]
and define $f_{i}: R_i \to W_i$ to act as $f_{M}$ on $U$ and on $L_i$ to send
\begin{itemize}
\item $k\mapsto r_p$ if 
\[
I(\gamma_i([m_{p}]))<k< I(\gamma_i([m_{p+1}]))
\]
\item $k\mapsto r_{min}$ if 
\[
k< I(\gamma_i([m_{p}]))
\]
for all $p\in \phi^{-1}(i)$
\item $k\mapsto r_{max}$ if 
\[
I(\gamma_i([m_{p}]))< k
\]
for all $p\in \phi^{-1}(i)$
\end{itemize}
We make $f_i$ into a morphism in $\Ass$ by taking the linear order induced by $L_i$ on the fibers over the $r_{p}$, $r_{min}$ and $r_{max}$. We then define 
\[
\overline{g}^i: f_Z^{-1}(i)\to R_i
\]
to act as $\coprod_{j\in \phi^{-1}(i)} \overline{g}_j$ on $\coprod_{j\in \phi^{-1}(i)}  I(\gamma_i([m_j]))$ and as the identity on $L_i$. We further define $\phi_i: W_i\to \{i\}$ to send every element to $i$. We thus have a commutative diagram 
\[
\begin{tikzcd}
\{i\}\arrow[Subseteq]{r}{} &\{i\} & \coprod_{j}I(\gamma_i([m_j]))\arrow[l,"f_{Z}"']\arrow[d,"\overline{g}^i"]\\
P\cap \phi^{-1}(i)\arrow[Subseteq]{r}{} & W_i\arrow[u,"\phi_i"] & R_i\arrow[l,"f_i"']
\end{tikzcd}
\]
in $\Ass$, which covers the morphism $\gamma_i:\bigoplus_{j\in \phi^{-1}(i)} [m_j] \to O(f_Z^{-1}(i))$. Taking the coproduct over $i\in \on{Im}(\phi)$ gives us a morphism
\[
\begin{tikzcd}
\on{Im}(\phi)\arrow[Subseteq]{r}{} &\on{Im}(\phi) & f_Z^{-1}(\on{Im}(\phi))\arrow[l,"f_{Z}"']\arrow[d,"\coprod_{i}\overline{g}^i"]\\
P\cap \phi^{-1}(i)\arrow[Subseteq]{r}{} & \coprod_{i}W_i\arrow[u,"\coprod_{i}\phi_i"] & \coprod_{i}R_i\arrow[l,"\coprod_{i}f_i"']
\end{tikzcd}
\]

Finally, we set
\[
W=(\coprod_{i\in \on{Im}(\phi)}W_i) \amalg (S\setminus \on{Im}(\phi))
\]
and 
\[
R=(\coprod_{i\in \on{Im}(\phi)}R_i) \amalg (T\setminus f_{Z}^{-1}(\on{Im}(\phi)))
\]
We then define morphisms:
\begin{itemize}
\item $g:W\to S$ to act as $\coprod_{i\in \on{Im}(\phi)} \phi_i$ on $\coprod_{i\in \on{Im}(\phi)} W_i$ and as the identity otherwise.
\item $f_{M,Z}: R\to W$ to act as $f_i$ on $R_i$ and as $f_Z$ on $T\setminus f_Z^{-1}(\on{Im}(\phi))$. 
\item $\overline{g}:T\to R$ to act as $\coprod_{i\in \on{Im}(\phi)} \overline{g}^{i}$ on $f_Z^{-1}(\on{Im}(\phi))$ and the identity elsewhere. 
\end{itemize}
By construction, this defines a commutative diagram
\begin{equation}\label{diag:MorphPhi}
\begin{tikzcd}
Q\arrow[Subseteq]{r}{}  & S & T\arrow[l,"f_{Z}"']\arrow[d,"\coprod_{i}\overline{g}"]\\
P\arrow[Subseteq]{r}{} & W\arrow[u,"g"] & R\arrow[l,"f_{M,Z}"']
\end{tikzcd}
\end{equation}
in $\Ass$, covering $(\phi,\{\gamma_i\})$, and the bottom row is in $\Omega_M$. We therefore define $X_{M,Z}$ to be the bottom row, and $\Phi$ to be the morphism defined by the diagram \eqref{diag:MorphPhi}. 

To check the remaining universal property, we 
let 
\[
P\subset A\overset{f_X}{\leftarrow} B
\]
and $\beta_i: O(f_X^{-1}(i))\cong [m_i]$ be another element in $\Omega_M^E$, and let $\nu$ be a morphism 
\begin{equation*}
\begin{tikzcd}
 Q\arrow[Subseteq]{r}{}& S & T\arrow[l, "f_Z"']\arrow[d, "\overline{\rho}"] \\
 P\arrow[Subseteq]{r}{}& A\arrow[u, "\rho"] & \arrow[l,"f_{X}"] B
\end{tikzcd}
\end{equation*}
covering $(\phi, \{\gamma_i\}_{i\in Q})$.

For each $i\in \on{Im}(\phi)$, the identity on $P$ and the condition nothing be sent to the basepoint uniquely determines a map of ordered sets 
\[
\zeta_i:\rho^{-1}(i)\to W_i.
\]
Moreover, the $\zeta_i$ together with the restriction of $\rho$ to $A\setminus \rho^{-1}(\on{Im}(\phi))$ uniquely determines a map 
\[
\zeta: A\to W
\]
such that the diagram 
\[
\begin{tikzcd}
A\arrow[rr,"\rho"]\arrow[dr,"\zeta"] & &  S \\
 & W\arrow[ur, "g"] &
\end{tikzcd}
\]
commutes. Note that $\zeta|_P$ induces the identity $P\to P$. 

Moreover, for each $i\in \on{Im}(\phi)$ the isomorphisms $I(\beta_i)$ on $I([m_j])$ and restriction $\overline{\rho}_i:L_i\to f_X^{-1}(\rho^{-1}(i))$  uniquely determine a map 
\[
\overline{\zeta}_i:R_i \to f_X^{-1}(\rho^{-1}(i)).
\]
These, together with the restriction of $\overline{\rho}$ to $T\setminus f_Z^{-1}(\on{Im}(\phi))$ uniquely determine a morphism 
\[
\overline{\zeta} R\to B
\]
such that the diagram 
\[
\begin{tikzcd}
B & & T\arrow[dl, "\overline{g}"]\arrow[ll,"\overline{\rho}"'] \\
 & R\arrow[ul,"\overline{\zeta}"] & 
\end{tikzcd}
\]
commutes, and the restriction of $\overline{\zeta}$ to $f_X^{-1}(P)$ is the isomorphism $\coprod_{i}I(\beta_i)$. 

We therefore have constructed a unique morphism 
\[
(\zeta,\overline{\zeta}):X_{Z,M} \to X
\]
in $\Omega_M^E$ such that the diagram 
\[
\begin{tikzcd}
 & Z\arrow[dr, "\Psi"]\arrow[dl,"\Phi"'] & \\
 X_{M,Z}\arrow[rr, "{(\zeta,\overline{\zeta})}"'] & & X
\end{tikzcd}
\]
commutes. 

\end{proof}
